1D and 2D Flow Routing on a Terrain

An important problem in terrain analysis is modeling how water flows across a terrain creating floods by forming channels and filling depressions. In this paper we study a number of \emph{flow-query} related problems: Given a terrain $\Sigma$, represented as a triangulated $xy$-monotone surface with $n$ vertices, a rain distribution $R$ which may vary over time, determine how much water is flowing over a given edge as a function of time. We develop internal-memory as well as I/O-efficient algorithms for flow queries. This paper contains four main results: (i) We present an internal-memory algorithm that preprocesses $\Sigma$ into a linear-size data structure that for a (possibly time varying) rain distribution $R$ can return the flow-rate functions of all edges of $\Sigma$ in $O(\rho k+|\phi| \log n)$ time, where $\rho$ is the number of sinks in $\Sigma$, $k$ is the number of times the rain distribution changes, and $|\phi|$ is the total complexity of the flow-rate functions that have non-zero values; (ii) We also present an I/O-efficient algorithm for preprocessing $\Sigma$ into a linear-size data structure so that for a rain distribution $R$, it can compute the flow-rate function of all edges using $O(\text{Sort}(|\phi|))$ I/Os and $O(|\phi| \log |\phi|)$ internal computation time. (iii) $\Sigma$ can be preprocessed into a linear-size data structure so that for a given rain distribution $R$, the flow-rate function of an edge $(q,r) \in \Sigma$ under the single-flow direction (SFD) model can be computed more efficiently. (iv) We present an algorithm for computing the two-dimensional channel along which water flows using Manning's equation; a widely used empirical equation that relates the flow-rate of water in an open channel to the geometry of the channel along with the height of water in the channel.

==> model.tex <==
\section{Flooding Model}
\header{Flow graph and flow functions.}
We transform $\mesh$ into a directed acyclic graph $\flowgraph$, 
referred to as the \textit{flow graph}, by directing each edge $\{u,v\}$ of $\mesh$ 
from $u$ to $v$ if $h(u) > h(v)$, and from $v$ to $u$ otherwise, i.e., 
each edge is directed in the downward direction. 
For each (directed) edge $(u,v)$, we define the \emph{local flow} $\localflow(u,v)$ 
to be the portion of water arriving at $u$ that flows along the edge $(u,v)$ to $v$. 
If $\localflow(u,v) = 0$, we can delete the edge $(u,v)$ from $\flowgraph$. 

The value of $\localflow(u,v)$ is, in general, based on relative heights of 
the downslope neighbors of $u$. 
Note that the SFD model has $\localflow(u,v) > 0$ for exactly one downslope neighbor of $u$. 
We will not focus on the specifics of the flow function used, and assume only
that it is specified and for a pair $u,v$ can be retrieved in $\BigO(1)$ time.

Following the edges of $\flowgraph$, water reaches a set of sinks of $\mesh$. 
We define a \textit{flow function} $\flow: \vertices^2 \to [0,1]$, 
which specifies the proportion of water that flows from a vertex $u$ to another vertex $v$. 
Recall that unlike the SFD model, water can flow from $u$ to $v$ along many paths. 
The flow function is defined recursively as follows:

\begin{equation}
    \flow(u,v) = 
    \begin{cases}
        \hfil 1 &\text{ if $u = v$,}\\
        \displaystyle\sum_{(u,w) \in \edges(\flowgraph)} \localflow(u,w) \cdot \flow(w,v) &\text{ otherwise.}
    \end{cases}
    \label{eqn:flow}
\end{equation}

For a maximal depression $\beta$, we define 

\begin{equation*}
    \flow(u,\beta) = \sum_{s \in \sinks(\beta)} \flow(u,s)
\end{equation*}
to be the portion of water that reaches from a vertex $u$ to $\beta$. 
Recall that $\sinks(\beta)$ is the set of sinks in $\beta$.

\header{Rain distribution.}
We let $\varregion(v): \vertices \to \mathbb{R}^{+}$ denote a \textit{rain distribution}, which is specified as 
a function on the vertices of the terrain, that is, for each vertex $v \in \vertices$, 
$\varregion(v) \geq 0$ indicates the rate at which it rains on $v$. 
We denote by $|\varregion|$ the number of vertices with positive rainfall in $\varregion$, 
and we assume that $\varregion$ is represented as a list of $|\varregion|$ pairs $(v,\varregion(v))$. 
In practice $|\varregion| \ll n$. 

Additionally, we can consider the distribution changing over time $\varregion(v,t): \vertices \times [0,t_{end}] \to \\mathbb{R}^+$ where $\varregion(v,t)$ specifies the rate at which it is raining at a given time $t$.  We will assume that for a each $v$, the distribution will be piecewise constant, with the function changing at $k$ values of $t$, and for all $v$  when $t \geq t_{end}$, $\varregion(v,t) = 0$. 

\header{Fill and spill rates.}
For a maximal depression $\beta$, we define the \textit{fill rate} 
$\fillrate_{\beta}: \reals_{\geq 0} \to [0,1]$ as the rate at which water is arriving in the depression $\beta$ 
as a function of time. 
That is, the rate at which rain is falling directly in $\beta$ 
plus the rate at which other depressions are spilling water into $\beta$. 
The fill rate $\fillrate_{\beta}$ is a monotonically nondecreasing piecewise-constant function. 
Similarly we define the \textit{spill rate} $\spillrate_\beta: \reals_{\geq 0} \to [0,1]$ 
as the rate (as a function of time) at which water spills from $\beta$ through the saddle that delimits $\beta$. 
Let $\filltime_{\beta}$, called the \textit{fill time}, be the time at which $\beta$ becomes full. 
Let $\beta'$ be the sibling depression of $\beta$. Then 
\begin{equation*}
    \spillrate_\beta(\vartime) = 
    \begin{cases}
        \hfil 0 
        &\text{ if $\vartime < \filltime_{\beta} \lor \filltime_{\beta'} \leq \filltime_{\beta}$,}\\
        \hfil \fillrate_\beta(\vartime) 
        &\text{ if $\vartime > \filltime_{\beta} \land \filltime_{\beta'} > \filltime_\beta$.}
    \end{cases}
\end{equation*}

By the definition of the fill rate, for any maximal depression $\beta$, its initial fill rate is
\begin{equation}
    \fillrate_{\beta}(0) = \sum_{s \in \sinks(\beta)} \sum_{v \in \vertices} \initrain(v) \flow(v,s),
    \label{eqn:initial-fillrate}
\end{equation}
which is how much rain water flows intially to the sinks of $\beta$. 
We can define $\fillrate_{\beta}(0)$ recursively using (\ref{eqn:flow}) as follows. 
Abusing the notation a little, let $\fillrate_{v}(0)$ denote the water reaching a vertex $v$ at time 0. 
Then 
\begin{align}
    \fillrate_{v}(0) &= \initrain(v)+\sum_{(w,v) \in \edges(\flowgraph)} \fillrate_w(0) \localflow(w,v) \label{eqn:dist-flow}\\ 
    \fillrate_{\beta}(0) &= \sum_{s \in \sinks(\beta)} \fillrate_{s}(0). \label{eqn:init-rate}
\end{align}

For any $\vartime \geq 0$ 
\begin{equation}
    \fillrate_{\beta}(t) = \fillrate_{\beta}(0)+\sum_{\alpha \in \tribs_\beta} \spillrate_{\alpha}(t) \flow(\saddle(\alpha), \beta).
    \label{eqn:fillrate}
\end{equation} 

That is, the fill rate of $\beta$ at time $\vartime$ is the direct rain reaching $\beta$ 
plus the water spilling into $\beta$ from its tributaries that are full. 

\header{Flow Function}
For an edge $e \in \terrain$, we define the \textit{flow rate} $\flowrate_{e}(t)$ as the rate at which water is passing along the edge as a function of time. 
We similarly define the flow rate of a vertex $v$ to be the sum of the flowrates along all downslope edges $(v,w)$. 

We can define $\flowrate$ as follows for any $\vartime \geq 0$,

\begin{align}
    \label{eqn:flowrate}
    \flowrate_v(t) &=  \initrain(v)+ \sum_{u \in \vertices} \initrain(u) \flow(u,v) +\sum_{\alpha \in \tribs_{\beta_v}} \spillrate_{\alpha}(t) \flow(\saddle(\alpha),v) \\
    \flowrate_{(u,v)}(t) &= \localflow(u,v)\flowrate_{u}(t) 
\end{align}

